Learning to Adapt the Parameters of Behavior Trees and Motion Generators (BTMGs) to Task Variations

The ability to learn new tasks and quickly adapt to different variations or dimensions is an important attribute in agile robotics. In our previous work, we have explored Behavior Trees and Motion Generators (BTMGs) as a robot arm policy representation to facilitate the learning and execution of assembly tasks. The current implementation of the BTMGs for a specific task may not be robust to the changes in the environment and may not generalize well to different variations of tasks. We propose to extend the BTMG policy representation with a module that predicts BTMG parameters for a new task variation. To achieve this, we propose a model that combines a Gaussian process and a weighted support vector machine classifier. This model predicts the performance measure and the feasibility of the predicted policy with BTMG parameters and task variations as inputs. Using the outputs of the model, we then construct a surrogate reward function that is utilized within an optimizer to maximize the performance of a task over BTMG parameters for a fixed task variation. To demonstrate the effectiveness of our proposed approach, we conducted experimental evaluations on push and obstacle avoidance tasks in simulation and with a real KUKA iiwa robot. Furthermore, we compared the performance of our approach with four baseline methods.

==> abstract.tex <==
The ability to learn new tasks and quickly adapt to different variations and dimensions is an important attribute in agile robotics. In previous work, we have explored Behavior Trees and Motion Generators BTMGs) as a robot arm policy representation to facilitate the learning and execution of assembly tasks. The current implementation of the BTMGs for a specific task may not be robust to the changes in the environment and  may not generalize well to different variations of tasks. To address this limitation, we propose to extend the BTMG policy representation by learning a modeling function that maps task variations to BTMG parameters. To achieve this, we first train a Gaussian process to predict performance measure or reward that takes BTMG parameters and task variations as input. We also train a classifier to check the feasibility of the predicted policy. Subsequently, we optimize the performance measure over BTMG parameters for a fixed task variation.
To demonstrate the effectiveness of our proposed approach, we conducted experimental evaluations on push and obstacle avoidance tasks in simulation and also performed physical experiments using a \textit{KUKA iiwa} robot. Furthermore, we compared the performance of our approach with four baseline methods.

==> table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{The median performance values and the $25^{th}$ and $75^{th}$ percentiles for both tasks. A "-" indicates that configuration was not evaluated.}
\label{tab:results}
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{|c|c|c|cc|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{Task} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Performance\\ Measure\end{tabular}} &
  \multirow{2}{*}{Environment} &
  \multicolumn{2}{c|}{Learned} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Optimized\\ GP\end{tabular}} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Nearest\\ Neighbor\end{tabular}} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Vanilla\\ GP\end{tabular}} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Single\\ Policy\end{tabular}} \\ \cline{4-13} 
 &
   &
   &
  \multicolumn{1}{c|}{Median} &
  Percentiles &
  \multicolumn{1}{c|}{Median} &
  Percentiles &
  \multicolumn{1}{c|}{Median} &
  Percentiles &
  \multicolumn{1}{c|}{Median} &
  Percentiles &
  \multicolumn{1}{c|}{Median} &
  Percentiles \\ \hline
\multirow{4}{*}{Obstacle} &
  \multirow{2}{*}{Total Reward} &
  Simulation &
  \multicolumn{1}{c|}{5050} &
  (4467, 5531) &
  \multicolumn{1}{c|}{\textbf{5013}} &
  (4290, 5462) &
  \multicolumn{1}{c|}{4834} &
  (3607, 5357) &
  \multicolumn{1}{c|}{4594} &
  (2635, 5143) &
  \multicolumn{1}{c|}{4496} &
  (-200, 5184) \\ \cline{3-13} 
 &
   &
  Reality &
  \multicolumn{1}{c|}{4963} &
  (4357, 5414) &
  \multicolumn{1}{c|}{\textbf{4966}} &
  (4238, 5426) &
  \multicolumn{1}{c|}{4782} &
  (3625, 5327) &
  \multicolumn{1}{c|}{--} &
  -- &
  \multicolumn{1}{c|}{--} &
  -- \\ \cline{2-13} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Finish Time\\ {[}sec{]}\end{tabular}} &
  Simulation &
  \multicolumn{1}{c|}{5.7} &
  (5.3, 7.3) &
  \multicolumn{1}{c|}{\textbf{5.9}} &
  (5.3, 7.5) &
  \multicolumn{1}{c|}{6.1} &
  (5.4, 12) &
  \multicolumn{1}{c|}{7} &
  (5.9, 12) &
  \multicolumn{1}{c|}{7.6} &
  (5.7, 12) \\ \cline{3-13} 
 &
   &
  Reality &
  \multicolumn{1}{c|}{5.8} &
  (5.4, 7.4) &
  \multicolumn{1}{c|}{\textbf{6.1}} &
  (5.4, 7.8) &
  \multicolumn{1}{c|}{6.1} &
  (5.5, 12) &
  \multicolumn{1}{c|}{--} &
  -- &
  \multicolumn{1}{c|}{--} &
  -- \\ \hline
\multirow{4}{*}{Push} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Position Error \\ {[}m{]}\end{tabular}} &
  Simulation &
  \multicolumn{1}{c|}{0.002} &
  (0.002, 0.003) &
  \multicolumn{1}{c|}{\textbf{0.006}} &
  (0.004, 0.009) &
  \multicolumn{1}{c|}{0.011} &
  (0.007, 0.083) &
  \multicolumn{1}{c|}{0.007} &
  (0.005, 0.014) &
  \multicolumn{1}{c|}{0.016} &
  (0.007, 0.123) \\ \cline{3-13} 
 &
   &
  Reality &
  \multicolumn{1}{c|}{0.01} &
  (0.007, 0.014) &
  \multicolumn{1}{c|}{\textbf{0.009}} &
  (0.007, 0.012) &
  \multicolumn{1}{c|}{0.016} &
  (0.01, 0.028) &
  \multicolumn{1}{c|}{--} &
  -- &
  \multicolumn{1}{c|}{--} &
  -- \\ \cline{2-13} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Orientation Error \\ {[}deg{]}\end{tabular}} &
  Simulation &
  \multicolumn{1}{c|}{0.15} &
  (0.07, 0.33) &
  \multicolumn{1}{c|}{\textbf{0.16}} &
  (0.07, 0.34) &
  \multicolumn{1}{c|}{0.18} &
  (0.08, 29.48) &
  \multicolumn{1}{c|}{0.11} &
  (0.06, 0.26) &
  \multicolumn{1}{c|}{0.29} &
  (0.1, 45.76) \\ \cline{3-13} 
 &
   &
  Reality &
  \multicolumn{1}{c|}{1.51} &
  (0.98, 2.76) &
  \multicolumn{1}{c|}{\textbf{1.42}} &
  (0.94, 2.74) &
  \multicolumn{1}{c|}{2.58} &
  (1.18, 6.23) &
  \multicolumn{1}{c|}{--} &
  -- &
  \multicolumn{1}{c|}{--} &
  -- \\ \hline
\end{tabular}%
}
\end{table*}

==> table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\begin{table}[]
\centering
\caption{Statistics to compute 100 task variations through RL-Pipeline. Numbers are in sec.}
\label{tab:learned}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|llllll}
\hline
Task     & Min   & Max     & Mean   & Median & \begin{tabular}[c]{@{}l@{}}Standard \\ Deviation\end{tabular}\\
\hline
Obstacle & 589.07 & 1342.56  & 788.908  & 736.175   & 171.251 \\
Push     & 1014.91  & 1310.12 & 1208.832 & 1207.04  & 62.915 \\
\hline
\end{tabular}%
}
\end{table}


==> table4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\begin{table}[]
\centering
\caption{Statistics to compute 100 task variations by optimizing the surrogate function. Numbers are in sec.}
\label{tab:optimization}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|llllll}
\hline
Task     & Min   & Max     & Mean   & Median & \begin{tabular}[c]{@{}l@{}}Standard \\ Deviation\end{tabular}\\
\hline
Obstacle & 0.611 & 76.269  & 6.439  & 1.317   & 13.401     \\
Push     & 1.964  & 129.293 & 31.806 & 10.958  & 37.582 \\
\hline
\end{tabular}%
}
\end{table}

